A Fourth-Order Cut-cell Multigrid Method for Solving Elliptic Equations on Arbitrary Domains

To numerically solve a generic elliptic equation on two-dimensional domains with rectangular Cartesian grids, we propose a cut-cell geometric multigrid method that features (1) general algorithmic steps that apply to two-dimensional constant-coefficient elliptic equations with both divergence and non-divergence forms and all types of boundary conditions, (2) the versatility of handling both regular and irregular domains with arbitrarily complex topology and geometry, (3) the fourth-order accuracy even at the presence of ${\cal C}^1$ discontinuities on the domain boundary, and (4) the optimal complexity of $O(h^{-2})$.Test results demonstrate the generality, accuracy, efficiency, robustness, and excellent conditioning of the proposed method.

==> sec/preliminaries.tex <==
\section{Preliminaries and notation}
\label{sec:preliminaries}

Two-dimensional (2D) continua
 with arbitrary topological structures and geometric features
 are modeled by the Yin space in \Cref{sec:yin-space}
 to furnish a Boolean algebra
 as well as a unique and efficient boundary representation.
Embedded inside a rectangle, 
 the complex domain is partitioned by the Boolean algebra
 into regular and irregular cells (or control volumes). 
% the latter of which contain the geometry of irregular boundaries. 
The contents in Subsections
 \ref{sec:PLG}, \ref{sec:LSP}, and \ref{sec:NC}
 concern finite-volume-based discretizations of continuous operators
 for these irregular cells. 

\subsection{Yin space}
\label{sec:yin-space}

In a topological space ${\mathcal X}$,
 the \emph{complement} of a subset ${\mathcal P}\subseteq {\mathcal X}$,
 written ${\mathcal P}'$,
 is the set ${\mathcal X}\setminus {\mathcal P}$.
% A subset of ${\mathcal X}$
%  is \emph{closed} if its complement is open.
The \emph{closure} of a set ${\mathcal P}\subseteq{\mathcal X}$,
 written $\overline{\mathcal P}$,
 is the intersection of all closed 
 supersets of ${\mathcal P}$.
The \emph{interior} of ${\mathcal P}$, written ${\mathcal P}^{\circ}$,
 is the union of all open subsets of ${\mathcal P}$.
% in ${\mathfrak T}$.
The \emph{exterior} of ${\mathcal P}$,
 written ${\mathcal P}^{\perp}:= {\mathcal P}^{\prime\circ}
 :=({\mathcal P}')^{\circ}$,
 is the interior of its complement.
% By the identity $\overline{\mathcal P} ={\mathcal P}^{\prime\circ\prime}$
%  \mbox{\cite[p. 58]{givant09:_introd_boolean_algeb}},
%  we have 
%  ${\mathcal P}^{\perp}={\mathcal P}^{-\prime}$.
A point $\mathbf{x}\in {\mathcal X}$ is
 a \emph{boundary point} of ${\mathcal P}$
 if $\mathbf{x}\not\in {\mathcal P}^{\circ}$
 and $\mathbf{x}\not\in {\mathcal P}^{\perp}$.
The \emph{boundary} of ${\mathcal P}$, written $\partial {\mathcal P}$,
 is the set of all boundary points of ${\mathcal P}$.
% It can be shown that
%  ${\mathcal P}^{\circ}={\mathcal P}\setminus \partial {\mathcal P}$
%  and
%  $\overline{\mathcal P}= {\mathcal P}\cup \partial {\mathcal P}$.

A subset $\calP$ in ${\cal X}$ is \emph{regular open}
 if it coincides with the interior of its closure.
%and is regular open iff $\calS = \calS^{\perp \perp}$. 
For $\calX = \bbR^2$, 
a subset $\calS \subset \bbR^2$ is \emph{semianalytic}
if there exist a finite number of analytic functions
$g_i : \bbR^2 \rightarrow \bbR$
such that $\calS$ is in the universe of a finite Boolean algebra
formed from the sets
$\calX_i = \left\{ \bmx \in \bbR^2 : g_i(\bmx) \ge 0 \right\}$. 
In particular, a semianalytic set is \emph{semialgebraic}
if all the $g_i$'s are polynomials. 
These concepts lead to 

\begin{definition}[Yin Space~\cite{Zhang2020:YinSets}]
  \label{def:yin-space}
  A \emph{Yin set} $\calY \subseteq \bbR^2$
   is a regular open semianalytic set 
   with bounded boundary.
  The Yin space $\bbY$ is
   the class of all Yin sets. 
\end{definition}

In \Cref{def:yin-space}, 
 the regularity captures the salient feature
 that continua are free of low-dimensional elements
 such as isolated points and crevices,  
 the openness leads to a unique boundary representation of any Yin set, 
 and the semianalyticity ensures that a finite number of entities
 suffice for the boundary representation.
%See~\cite{Zhang2020:YinSets} for more explanations.
More precisely,
 each Yin set $\calY \neq \emptyset, \bbR^2$
 can be uniquely expressed \cite[Corollary 3.13]{Zhang2020:YinSets} as
\begin{equation}
  \calY = \bigcup\nolimits_{j} {}^{\perp\perp} {\cal Y}_i
  = \bigcup\nolimits_{j} {}^{\perp\perp}
  \bigcap\nolimits_{i} \intr(\gamma_{j, i}),
\end{equation}
where ${\cal Y}_j$ is the $j$th connected component of $\calY$,
$\{\gamma_{j,i}\}$ 
the set of pairwise almost disjoint Jordan curves
satisfying $\partial {\cal Y}_i=\cup_j\gamma_{j,i}$, 
%$\gamma$ an oriented Jordan curve,
and $\intr(\gamma_{j,i})$ the complement of $\gamma_{j,i}$
that always lies at the left of an observer
who traverses $\gamma_{j,i}$ according to its orientation.
% The whole collection $\{\gamma_{j,i}\}$
% can be further arranged in a fashion
% such that the topological information (such as Betti numbers)
% can be easily extracted within constant time;
% see~\cite[Definition 3.17]{Zhang2020:YinSets}.

\begin{theorem}[Zhang and Li~\cite{Zhang2020:YinSets}]
  \label{thm:booleanAlgebra}
  Define the regularized union operation $\cuppp$
  as $\calS \cuppp \calT := \left(\calS \cup \calT \right)^{\perp \perp}$. 
  Then $\left(\bbY, \cuppp, \cap, ^\perp, \emptyset, \bbR^2 \right)$
  is a Boolean algebra.
\end{theorem}
% It can be shown~\cite[\S 10]{Givant:BooleanAlgebra} that
% the class of all regular open subsets of $\calX$
% is closed under the regularized union. 

\begin{corollary}
  \label{coro:booleanAlgebra}
  Denote by $\bbY_{\mathrm{c}}$ the subspace of $\bbY$
  where the boundary of each Yin set 
  is constituted by a finite number of cubic splines.
  Then $\bbY_{\mathrm{c}}$ a sub-algebra of $\bbY$. 
\end{corollary}

The Boolean algebra in \Cref{coro:booleanAlgebra}
 are implemented 
 in~\cite[Section 4]{Zhang2020:YinSets}
 and employed in this work
 to cut and merge cells; see \Cref{sec:grid}.

%Developed in \cite{Zhang2020:YinSets} alongside the notion of Yin space 
%In \cite{Zhang2020:YinSets}
%the authors developed (1) a simple representation scheme of Yin sets
%that facilitates geometric and topological queries, and
%(2) the efficient algorithms implementing the Boolean operations
%in Theorem \ref{thm:booleanAlgebra}.
%The cut cell construction in this work will be based on these results.

\subsection{Poised lattice generation}
\label{sec:PLG}

Traditional finite difference (FD) methods
have limited applications in irregular domains,
as they often replace the spatial derivatives in partial differential equations 
by one-dimensional FD formulas or their tensor-product counterparts.
To overcome this limitation,
the PLG algorithm~\cite{Zhang:PLG} was proposed 
to generate poised lattices in complex geometries.
Once the interpolation lattices have been generated,
high-order discretization of the differential operators can be obtained
via multivariate polynomial fitting.

In this section we give a brief review of the PLG problem.
We begin with the relevant notions in multivariate interpolation.
\begin{definition}[Lagrange interpolation problem (LIP)]
Denote by $\Pi_n^{\Dim}$ the vector space of 
all $\Dim$-variate polynomials of degree no more than $n$
with real coefficients. 
Given a finite number of points $\bmx_1, \bmx_2, \cdots, \bmx_N \in \bbR^\Dim$
and the same number of data $f_1, f_2, \cdots, f_N \in \bbR$, 
the \emph{Lagrange interpolation problem} seeks a polynomial $f \in \Pi_n^\Dim$ such that
\begin{equation}
f(\bmx_j) = f_j, \quad \forall j=1, 2, \cdots, N, 
\label{eq:finiteDiffLIP}
\end{equation}
where $\Pi_n^\Dim$ is the \emph{interpolation space} 
and $\bmx_j$'s the \emph{interpolation sites}. 
\label{def:finiteDiffLIP}
\end{definition}

%In the above Definition, 
The sites $\left\{ \bmx_j \right\}_{j=1}^N$ are said to be \emph{poised} in $\Pi_n^\Dim$
if there exists a unique $f \in \Pi_n^\Dim$ satisfying (\ref{eq:finiteDiffLIP})
for any given data $\left\{ f_j \right\}_{j=1}^N$. 
Suppose $\left\{ \phi_j \right\}$ is a basis of $\Pi_n^\Dim$.
It is easy to see that the interpolation sites are poised
if and only if $N = \dim \Pi_n^\Dim = \binom{n+\Dim}{n}$
and the $N \times N$ \emph{sample matrix}
\begin{equation}
M(\left\{ \phi_j \right\} ; \left\{ \bmx_k \right\}) = \Big[ M_{jk} \Big] := \Big[ \phi_j(\bmx_k) \Big]
\quad (1 \le j, k \le N)
\label{eq:sampleMatrix}
\end{equation}
is non-singular. 

\begin{definition}[PLG in $\mathbb{Z}^\Dim$~\cite{Zhang:PLG}]
\label{def:PLG}
    Given a finite set of feasible nodes $K\in \mathbb{Z}^\text{D}$, 
	 a starting point $\mathbf{q}\in K$, and a degree $n\in \mathbb{Z}^+$,
	 the \emph{problem of poised lattice generation} is to
	 choose a lattice $\mathcal{T}\subset K$ such that 
	 $\mathcal{T}$ is poised in $\Pi_n^\Dim$ and $\#\mathcal{T} = \dim \Pi_n^\Dim$.
\end{definition}

In \cite{Zhang:PLG}, we proposed a novel and efficient PLG algorithm to 
 solve the PLG problem via an interdisciplinary research of approximation theory,
 abstract algebra, and artificial intelligence.
The stencils are based on the transformation of the principal lattice.
In this work, we directly apply the algorithm to our finite volume discretization.
The starting point $\mathbf{q}$ corresponds to the cell index 
at which the spatial operators are discretized,
 and the feasible nodes $K$ formed by collecting the indices of nearby cut cells.
 
In general cases it is still unclear that
 whether a direct application of the PLG algorithm
 will generate poised stencils in finite volume formulation.
Finding a strict proof of poisedness %of the generated stencils % in the finite volume sense
 will be a topic of our future research.
Nevertheless, the poisedness in finite volume formulation is supported
 by the extensive numerical evidences.
For example, the condition numbers of the $(\Dim,n) = (2,4)$ lattices used in this paper
generally do not exceed $10^4$ in all problems of interest.

\subsection{Least squares problems}
\label{sec:LSP}

To derive the approximation to the differential operators,
we need the following results on weighted least squares fitting.

\begin{definition}
For a symmetric positive definite matrix $W \in \bbR^{n \times n}$, 
the \emph{$W$-inner product} is
\begin{equation}
\langle u, v \rangle_W := u^T W v
\end{equation}
and the \emph{$W$-norm} is
\begin{equation}
\Vert u \Vert_W := \langle u, u \rangle_W^{1/2}
\end{equation}
for $u, v \in \bbR^n$. 
\end{definition}

\begin{proposition}
Let $A \in \bbR^{m \times n}$ be a matrix with full column rank,  and let %$b \in \bbR^m$, 
$W \in \bbR^{m \times m}$ be a symmetric positive definite matrix. 
%Denote by $W^{1/2}$ the square root of $W$. 
\begin{enumerate}[label={(\roman*)}, nosep, leftmargin=*]
\item For any $b \in \bbR^m$, the optimization problem
%If $A$ has full column rank, then the optimization problem
\begin{equation}
\min_{x \in \bbR^n} \left\Vert Ax - b \right\Vert_{W}
\end{equation}
admits a unique solution $x_{\mathrm{LS}} = \left(A^T W A\right)^{-1} A^T W b$. 
\item For any $d \in \bbR^n$, the constrained optimization problem
%If $A$ has full row rank, then the constrained optimization problem
\begin{equation}
\min_{x \in \bbR^m} \left\Vert x \right\Vert_{W^{-1}} \quad \mathrm{s.t.} \quad A^T x=d
\end{equation}
admits a unique solution $x_{\mathrm{NM}} = W A \left(A^T W A\right)^{-1} d$. 
\end{enumerate}
\label{prop:leastSquares}
\end{proposition}
\begin{proof}
See~\cite[\S 5.3, \S 5.6, \S 6.1]{Golub}.
\end{proof}

\subsection{Numerical cubature}
\label{sec:NC}

In finite volume discretization,
we need to evaluate the volume integral
%$\int_{\calC} f \rmd \bmx$
of a given function $f(x, y)$ over a control volume
$\calC \in \bbY_{\mathrm{c}}$. 
%$\calC \subset \bbR^2$. 
For this purpose, 
we invoke the Green's formula to convert
\begin{equation}
%\int_{\calC} f \rmd \bmx = 
\iint_{\calC}  f(x, y) \rmd x \rmd y
= \oint_{\partial \calC} F(x, y) \rmd y
\label{eq:volumeIntegral}
\end{equation}
into a line integral, 
where $\partial \calC$ is the boundary of $\calC$ and 
$F(x, y) = \int_{\xi_0}^{x} f(\xi, y) \rmd \xi$
is a primitive of $f(x, y)$ with respect to $x$,
with $\xi_0$ an arbitrary fixed real number.
Suppose $\left( x(t), y(t) \right) \left( t \in [0,1] \right)$
is a smooth parametrization of $\partial \calC$. 
Then we can write %the integral (\ref{eq:volumeIntegral}) can be recasted into
\begin{subequations}
\begin{align}
 \oint_{\partial \calC} F(x, y) \rmd y &= \int_0^1 F(x(t), y(t)) \dot{y}(t) \rmd t \\
&=  \int_0^1\dot{y}(t) \int_{\xi_0}^{x(t)} f(\xi, y(t)) \rmd \xi  \rmd t, 
\label{eq:iteratedIntegral}
\end{align}
\end{subequations}
into a two-fold iterated integral. 
The integral (\ref{eq:iteratedIntegral}) 
can be evaluated using one-dimensional numerical quadratures 
such as Gauss-Legendre quadrature.
%the composite Newton-Cotes formulas, 
%and the adaptive Simpson rule. 
If the boundary $\partial \calC$ is only piecewise smooth, 
we simply apply (\ref{eq:iteratedIntegral}) to each piece and sum up the results.
If the integrand $f(x, y)$ is a bivariate polynomial, %and $\partial \calC$ is represented by splines, 
then (\ref{eq:iteratedIntegral}) expands to a (possibly very high-order) polynomial of $t$
whose coefficients depend on the parametrization $\left( x(t), y(t) \right)$ and the integrand $f(x, y)$. 
This polynomial can then be evaluated to machine precision without quadratures.

Although $\xi_0$ can be arbitrary, 
it should be selected to minimize round-off errors. 
A typical choice is the center of the bounding box of $\calC$.
See~\cite{Sommariva} for a detailed error analysis
on using Gauss-Legendre quadrature to evaluate the cubature formula (\ref{eq:iteratedIntegral}).
%\begin{remark}
%(1) Although $\xi_0$ can be arbitrary, 
%it should be selected to minimize round-off errors. 
%A typical choice is the center of the bounding box of $\calC$. 
%(2) %When using numerical quadratures to evaluate (\ref{eq:iteratedIntegral}), 
%The quadrature nodes do not necessarily lie in $\calC$ nor on $\partial \calC$. 
%(3) See~\cite{Sommariva} for a detailed error analysis
%on using Gauss-Legendre quadrature to evaluate the cubature formula (\ref{eq:iteratedIntegral}). 
%\end{remark}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../ellipticFV2D"
%%% End:

% LocalWords:  semianalytic

